A Sampling Theorem for Deconvolution in Two Dimensions

This work studies the problem of estimating a two-dimensional superposition of point sources or spikes from samples of their convolution with a Gaussian kernel. Our results show that minimizing a continuous counterpart of the $\ell_1$ norm exactly recovers the true spikes if they are sufficiently separated, and the samples are sufficiently dense. In addition, we provide numerical evidence that our results extend to non-Gaussian kernels relevant to microscopy and telescopy.

==> withheld.tex <==
\begin{figure}[t!]
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics{fig/nearpoint1D.pdf}
\caption{}
\label{fig:nearpoint1D}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics{fig/distantpoint1D.pdf}
\caption{}
\label{fig:distantpoint1D}
\end{subfigure}\vspace{.15in}\\
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics{fig/nearpoint2D.pdf}
% \caption{}
% \label{fig:nearpoint2D}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics{fig/distantpoint2D.pdf}
% \caption{}
% \label{fig:distantpoint2D}
% \end{subfigure}\vspace{.15in}\\
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics{fig/hex6.pdf}
\caption{}
\label{fig:hex6.pdf}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics{fig/hex7.pdf}
\caption{}
\label{fig:hex7.pdf}
\end{subfigure}
\caption[Spike Separations in 1D and 2D]{Differences in spike positions in one dimension versus higher dimensions.}
\label{fig:neardistant}
\end{figure}


It is clear in one dimension that if an interpolating $Q$ exists for all supports $T$ with minimum separation $\spikesep(T)$ where $\abs{Q(t)}<1$ for $t$ within $\spikesep(T)/2$ of $T$, 
%$\abs{Q(t)}<1$ holds for all $t$ within $\spikesep(T)/2$ of support $T$ uniformly for all $T$ with minimum separation $\spikesep(T)$,
then $\abs{Q(t)}<1$ should hold for farther $t$ too.
%Additional space beyond $\spikesep(T)/2$ between $t$ and its nearest spike pushes the positions of all other spikes down the axis.
\Cref{fig:nearpoint1D} depicts this where a generic point $t$ (in blue) is less than $\spikesep(T)/2$ from spikes (in red) in $T$. The blue perimeter depicts this separation and does not affect the separation between other spikes. 
In \Cref{fig:distantpoint1D} where $t$ (in blue) is farther than $\spikesep(T)/2$ from the nearest spike, this extra separation beyond $\spikesep(T)/2$ is also added to its distance from every other spike.
Then the Gaussian components of $Q$ that surround each spike will decay more over the extra distance to $t$, ensuring the bound. 

However in two dimensions there is no simple argument to show that additional space between $t$ and its nearest spike pushes every other spike away from $t$.
% To see this in \Cref{fig:nearpoint2D}, $t$ (in blue) is within $\spikesep(T)/2$ of a spike at the origin, and the blue circle delimiting this separation does not impinge on the positions of other nearby spikes.
% But if $t$ is a point farther than $\spikesep(T)/2$ from support $T$, as is the blue point depicted in \Cref{fig:distantpoint2D}, this extra separation affects surrounding spikes.
% Those spikes (in gray) enclosed by the circle, which indicates the distance of the nearest spike, are pushed to points outside the circle shown in green.
The effect this has on all farther spikes is not clear and so it is not as simple to bound $Q$ in this case.
We provide a particular example of this in \Cref{fig:hex6.pdf} which shows a dense packing of seven spikes, where a point $t$ sits $\spikesep(T)/2$ away from its nearest spike and is surrounded by three others.
In \Cref{fig:hex7.pdf} one spike is removed making room for two more to take its place.
There the point $t$ sits farther than $\spikesep(T)/2$ from any spike but since it sits closer to five nearby spikes it is not clear that an interpolating $Q$ bounded near $T$ is also bounded at $t$.
Thus \Cref{lem:QBoundFar} requires a stronger argument.

%This perimeter is already contained in the circle of radius $\spikesep(T)$ about the origin.
%Since spikes in all other hexagonal cells must sit at least $\spikesep(T)$ from the central spike as indicated that image, the contributions from them to $Q(t)$ will be less at $t$ on account of this extra space.

% For $t$ within $\spikesep(T)/2$ of a spike, its proximity to the spike provides it some protection in a sense, limiting the number of other spikes that can be near it.
% In two dimensions, leaving this perimeter potentially puts it closer to more elements of the support so while an interpolating $Q$ might be less than 1 within a $\spikesep(T)/2$ of the support we need a stronger argument than monotonicity to show that it satisfies \eqref{eq:conditionQTc} everywhere off the support.
% That is we cannot rely on a monotonicity argument in this case to guarantee that a dual certificate can be constructed. 

%The spikes previously positioned at the four gray points must move outside the blue circle (indicating distance to the nearest spike) as the green points are.


%As mentioned earlier, in two and higher dimensions \Cref{lem:QBoundFar} is not a corollary of \Cref{lem:QBoundNear} since keeping $t$ within $\spikesep(T)/2$ of a spike prevents other spikes from being close to $t$.
Instead we prove \Cref{lem:QBoundFar} by deriving lower bounds on the distances to nine of the nearest spikes from an arbitrary point $t$ that lies farther than $\spikesep(T)/2$ from the support $T$.
Since $Q$ is a sum of Gaussians centered near each spike, it decays rapidly away from $T$.
Thus most of $Q(t)$ comes from bumps and waves near $t$, so giving precise distance limits for these spikes sharpens $\abs{Q}$'s bound.
We split into multiple cases the locations of two of the nearest spikes from $t$, then show how each case affects the proximity to $t$ of adjacent spikes.
By choosing small regions for the locations of the first two spikes and using the separation constraints, we can sharpen bounds on other spike's distances to show $\abs{Q(t)}<1$ for choices of $\spikesep(T)$ and $\gridsep$. 

Suppose $t$ is at least $\spikesep(T)/2$ from $T$.
If $t$ is the origin then at most nine spikes lie in the numbered cells in \Cref{fig:CellNumber}.
We denote $U_i$'s spike as $t_i$.
The next lemma provides lower bounds on the distance from $t$ of spikes in $U_1$ through $U_9$ provided each $U_i$ contains a spike. We use these to bound $\abs{Q(t)}$.

\begin{figure}[t]
\centering
\includegraphics{fig/CellNumber.pdf}
\caption[Cell Numbering]{\label{fig:CellNumber}Cell indices for \Cref{lem:Norms9}}
\end{figure}

\begin{lemma}[Proof in \Cref{sec:Norms9Proof}]\label{lem:Norms9}
Suppose a signal with support $T$ has minimum separation $\spikesep(T)$, and the origin is at least $\spikesep(T)/2$ away from any spike.
Let $t_1$ be the nearest spike from the origin and orient the positive horizontal axis to pass through $t_1$.
Let $t_2\in U_2$ sit in the upper half plane.
Denote by $t_i$ the spike in $U_i$ depicted in \Cref{fig:CellNumber}.
If $t_1=(t_1^{(1)},0)$ % sits on the segment between $(l_1,0)$ and $(r_1,0)$ and 
and $t_2=(t_2^{(1)},t_2^{(2)})$
with $\spikesep(T)/2\leq l_1\leq t_1^{(1)}\leq r_1\leq \spikesep(T)$ and $l_2\leq t_2^{(1)}\leq r_2$ where $(l_2,0),(r_2,0)\in U_2$,
then the following holds:
\begin{gather}
\norm{t_1},\norm{t_4}\geq l_1,\quad
\norm{t_2}\geq\max(\abs{r_2},l_1),\label{eq:t2}\\
\norm{t_3}\geq \max\left(l_1, \sqrt{\max(0,\Delta^2-l_2^2)}\right),\label{eq:t3a}\\
%\norm{t_3}\geq \norm{z} \quad\text{for any $z\in\RR^2$ with}\quad \norm{z-(r_1,0)}=\spikesep(T)\text{~and~}\norm{z-(l_2,0)}=\spikesep(T),\label{eq:t3}\\
\norm{t_5},\norm{t_6}\geq\max\left(l_1,\sqrt{\spikesep(T)^2-r_1^2}\right),\label{eq:t5t6}\\
\norm{t_7},\norm{t_8}\geq\norm{(y_1,y_2)}\mbox{ s.t. }y_1=\sqrt{3}\spikesep(T)/2,\ y_2=
\begin{cases}
\sqrt{\spikesep(T)^2-(\sqrt{3}\spikesep(T)/2-l_1)^2} & \frac{l_1+r_1}{2}\leq\frac{\sqrt{3}\spikesep(T)}{2},\\
\sqrt{\spikesep(T)^2-(\sqrt{3}\spikesep(T)/2-r_1)^2} & \frac{l_1+r_1}{2}\geq\frac{\sqrt{3}\spikesep(T)}{2},
\end{cases}\\
\norm{t_9}\geq\norm{(y_1,y_2)}\ \mbox{s.t.}\ (y_1-l_1)^2+y_2^2=\spikesep(T)^2,\ y_2=
\begin{cases}
\frac{y_1}{\sqrt{3}}-\frac{\spikesep(T)}{2} & l_1\leq \frac{\sqrt{3}\spikesep(T)}{2},\\
-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep(T)}{2} & l_1\geq \frac{\sqrt{3}\spikesep(T)}{2}.
\end{cases}
\end{gather}
\end{lemma}

Note these bounds are particular to each $U_i$ and do not hold for other cells in symmetric positions. That is, the bound on $U_9$ does not hold for the cell left of $U_2$ despite their similar relative positions to the origin. Should any of $t_1$ through $t_9$ be absent, $\abs{Q(t)}$ will be smaller which we explain in the proof of \Cref{lem:QBoundFar}. Thus it is fine to assume each exists.

We use the bounds from \Cref{lem:Norms9} to solve \Cref{lem:QBoundFar} by considering different cases for $l_1$, $r_1$, $l_2$ and $r_2$.
We partition the horizontal axis between $(.5\spikesep(T),0)$ and $(\spikesep(T),0)$ into intervals of length $.05\spikesep(T)$ and consider each a different case for $[l_1,r_1]$.
We do the same for $t_2$ within $U_2$ by considering multiple cases for $[l_2,r_2]$.
\Cref{lem:Norms9} simplifies a range of positions for $t_1$ and $t_2$ into a single bound for each $\norm{t_i}$.
Thus a finite number of cases for $[l_1,r_1]$ and $[l_2,r_2]$ produce a finite number of cases for lower bounds on $\norm{t_1}$ through $\norm{t_9}$.
%\Cref{lem:Norms9} simplifies a range of positions for $t_1$ and $t_2$ into a finite number of cases for $[l_1,r_1]$ and $[l_2,r_2]$, each with a single bound for each $\norm{t_i}$.
%Thus there are a finite number of cases for the lower bounds on $t_1$ through $t_9$.
%\cfg{here you should mention why it's fine to assume that $t_2$ exists (I know it's somewhere else)}
Smaller intervals for $t_1$ and $t_2$ produce larger excluded regions so better bounds can be obtained by shrinking the partition intervals $[l_1,r_1]$ and $[l_2,r_2]$ and considering more cases.
These lower bounds on $\norm{t_i}$ are used in the proof of \Cref{lem:QBoundFar}.
%Additional improvements might be made by considering positions for spikes $t_3$ and higher but we leave that for later work.


\begin{proof}[Proof of \Cref{lem:QBoundFar}]
%\cfg{do you explain somewhere why it's fine to evaluate a finite number of values for l1, r1...? I imagine it's a similar argument to what we do when evaluating the bounds}
If $d_i$ is a sequence such that $d_i\leq\norm{t_i-t}$, by monotonicity of $\enva{B}$ and $\enva{W^k}$ an obvious upper bound on $\abs{Q(t)}$ is
\begin{equation}\label{eq:QBound}
\abs{Q(t)}\leq\sum_{i=1}^\infty \norminf{\bcoeff}\enva{B}(d_i)+\norminf{\wocoeff}\enva{W^1}(d_i)+\norminf{\wtcoeff}\enva{W^2}(d_i).
\end{equation}
Without loss of generality we assume $t$ sits at the origin.
Since $t_1$ is the nearest spike it must exist.
We assume here that $t_2$ exists in $U_2$.
In the case that $t_2$ is absent, letting $\norm{t_3}=l_1$ yields a smaller sum bounding $\abs{Q}$ than that in \Cref{lem:Norms9} when $\norm{t_2}=l_1$.
Thus if $\abs{Q}<1$ when $t_2$ exists, it also holds when it does not.
Spike positions in \Cref{lem:Norms9} only depend on $t_1$ or $t_2$, so the absence of any other spike will not affect $\norm{t_i}$ and so will only produce a smaller sum for \eqref{eq:QBound}.
%\cfg{not sure what you mean}

When $\spikesep(T)/2\leq\norm{t_1}\leq\spikesep(T)$, \Cref{lem:Norms9} establishes lower bounds on distances $\norm{t_1}$ through $\norm{t_9}$ for different cases of $t_1$ and $t_2$.
For spikes from other nearby cells ($U_i$ for $i>9$) we use the distance of the cell from the origin in \eqref{eq:QBound}, i.e. $u_i$ in \Cref{lem:normbound} which do not depend on other $t_i$.
%\bdb{It also feels like we are missing a figure showing the result of calculations occurring behind the scenes.}
When $\norm{t_1}\geq\spikesep(T)$ we let $\norm{t_i}=\spikesep(T)$ for $i=1$ through 6, and let $\norm{t_i}=u_i$ for $i>6$.
Contributions from distant spikes (ninth layer and beyond) are less than $\epsbump$ and $\epswave$ by \Cref{lem:BumpTail}.
In supplementary code we compute the sum \eqref{eq:QBound} for each case of $[l_1,r_1]$ and $[l_2,r_2]$ and show $\abs{Q(t)}<1$ in all cases for the choices of $\spikesep(T)$ and $\gridsep$ in the blue shaded region in \Cref{fig:FarQMap}. The choices of $(\spikesep(T),\gridsep)$ satisfying \Cref{lem:QBoundNear} (orange region in \Cref{fig:FarQMap}) are contained in this region.
\end{proof}

\begin{figure}
%\begin{subfigure}{\textwidth}%{0.5\textwidth}
\centering
\includegraphics[scale=0.5]{asy/FarRecoveryMap.jpg}
%\caption{\label{fig:FarQMap}}
%\end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \centering
% \includegraphics[scale=0.5]{asy/RecoveryMap.jpg}
% \caption{\label{fig:ExactRecoveryRegion}}
% \end{subfigure}
 \caption[Exact Recovery Regions]{The blue shaded region indicates choices of $\spikesep(T)$ and $\gridsep$ for which $\abs{Q(t)}<1$ for $t$ that are farther than $\spikesep(T)/2$ from every spike, and overlaid in orange are the parameter choices for $\spikesep(T)$ and $\gridsep$ in which we have proven $\abs{Q}<1$ within $\spikesep(T)/2$. Since this is contained in the blue, this region is where $\abs{Q}<1$ for all points outside the support.}
 \label{fig:FarQMap}
\end{figure}

The orange shaded region in \Cref{fig:FarQMap} indicates the parameters for which $\abs{Q}<1$ for both $t$ less than $\spikesep(T)/2$ from any spike and for $t$ farther than $\spikesep(T)/2$ from all spikes.
Thus $\abs{Q(t)}<1$ for $t$ outside the spike support $T$. Thus the existence of a valid interpolating function $Q$ is confirmed for these $(\spikesep(T),\gridsep)$ depicted in \Cref{fig:RecoveryMapFirst} and \Cref{thm:Exact} is resolved by \Cref{prop:DualCert}.


\subsection{Proof of \Cref{lem:Norms9}}\label{sec:Norms9Proof}

We introduce two lemmas we rely on before presenting the proof:

\begin{restatable}[Proof in \Cref{sec:ConvexIntersectProof}]{lemma}{ConvexIntersect}\label{lem:ConvexIntersect}
If $S$ is a convex set and $S+y=\{x+y:x\in S\}$ then $\bigcap_{c\in\conv(\{a_i\})}S+c=\bigcap_{i=1}^n S+a_i$, where $a_1,\ldots,a_n\in\RR^2$ and $\conv$ denotes the convex hull.
In particular, if $I$ is the line segment in $\RR^2$ between points $l$ and $r$, then
\begin{equation}
\bigcap_{x\in I}S+x= S+r\cap S+l.
\end{equation}
\end{restatable}
\begin{restatable}[Proof in \Cref{sec:ConvMinProof}]{lemma}{convmin}\label{lem:convmin}
Let $A\subset\RR^2$ be convex and closed and $B\subset\RR^2$ such that $A\setminus B \neq\emptyset$.  Then
\begin{equation}
\inf_{v\in A\setminus B}\|v\|^2
=
\begin{cases}
\|v^*\|^2 & \text{if $v^*\notin B$,}\\
\inf_{v\in \brac{\overline{A\setminus B}}\cap\partial B}\|v\|^2 & \text{otherwise,}
\end{cases}
\end{equation}
where $v^*=\argmin_{v\in A}\|v\|^2$, $\partial B$ denotes the boundary of $B$, and $\overline{A\setminus B}$ denotes the closure of $A\setminus B$.
\end{restatable}

\begin{proof}[Proof of \Cref{lem:Norms9}]
Without loss of generality assume $t_1$, the spike nearest to the origin, sits on the positive horizontal axis. Any other arrangement can be viewed as a rotation of one satisfying this.
Additionally we assume that $t_2$ lies above the horizontal axis in $U_2$ since other spike arrangements with $t_2$ below are a reflection and the same bounds can be shown.
We label spikes according to the numbered cells in \Cref{fig:CellNumber} with spike $t_i$ in $U_i$.
Note that hexagon edges have length $\spikesep(T)/2$ since each $U_i$ has diameter $\spikesep(T)$.
Let $B_{l_1}=\{t:\norm{t}< l_1\}$ with boundary $\partial B_{l_1}$.
%\bdb{if we are assuming all spikes exist, we should state this, or be clear about the situation}.
%\Cref{fig:.5Spike} and \Cref{fig:.65Spike} show the nearest possible locations for spikes in $U_2$ through $U_9$ when fixing the position of $t_1$, with $\norm{t_1}=.5\spikesep(T)$ and $\norm{t_1}=.65\spikesep(T)$ respectively.

%The nearest point to the origin in each cell outside the red or black circles ($y\in H_i$ such that $\norm{y-x_1}\geq\spikesep(T)$ and $\norm{y}\geq\norm{x_1}$) lies on one of the circle's border. Any other point will be an interior pointse else a nearer point can be found by reducing one of the two coordinates 
 
%As an example of our approach, \Cref{fig:.5Spike} depicts a scenario where the nearest spike $x_1=(\spikesep(T)/2,0)$. Note that hexagon edges have length $\spikesep(T)/2$ since each hexagon has a diameter of $\spikesep(T)$. The blue points depict the points nearest to the origin in the surrounding cells that are at least $\spikesep(T)$ from $x_1$, i.e. the worst case scenarios for $x_i$ given $x_1$, which occurs at the leftmost intersection of the red circle with each hexagon by \Cref{lem:CircleDist}. The black circle about the origin has radius $\spikesep(T)/2$ or $d_1=\norm{x_1}$. Obviously no other spike sits closer than $x_1$ the nearest.

%Since we cannot determine whether this placement of $x_1$ yields the worst case scenario, we must also consider arrangements where $d_1$ is larger. If $x_1$ is moved to the right slightly then the picture changes. \Cref{fig:.65Spike} shows another example with $x_1=(.65\spikesep(T),0)$. The black circle, with radius $d_1=.65\spikesep(T)$, pushes $x_2$, $x_3$, and $x_4$ out off the red circle, while the other points either move slightly closer or farther from the origin as the red circle moves to the right with $x_1$.

\begin{figure}[!t]
\centering
\begin{subfigure}[h]{0.3\textwidth}
\centering
\includegraphics{fig/point5Spike.pdf}
\caption{\label{fig:.5Spike}}
\end{subfigure}
\begin{subfigure}[h]{0.3\textwidth}
\centering
\includegraphics{fig/point65Spike.pdf}
\caption{\label{fig:.65Spike}}
\end{subfigure}
\begin{subfigure}[h]{0.3\textwidth}
\centering
\includegraphics{fig/IntersectSpike.pdf}
\caption{\label{fig:IntersectSpike}}
\end{subfigure}
\caption[Spike Perturbations]{
\Cref{fig:.5Spike} depicts a scenario where the nearest spike $t_1=(\spikesep(T)/2,0)$.
The blue points indicate the nearest points from the origin in cells 2 through 9 that are at least $\spikesep(T)$ from $t_1$, i.e. lower bounds for $\norm{t_i}$ given $t_1$, which occurs at the leftmost intersection of the red circle with each hexagon by \Cref{lem:CircleDist}.
The black circle depicts $\partial B_{l_1}$ where $\norm{t_1}=l_1=\spikesep(T)/2$.
By construction no other spike sits within $B_{l_1}$.
%Since we cannot determine whether this placement of $t_1$ yields the worst case scenario, we must also consider arrangements where $d_1$ is larger.
%If $t_1$ is moved to the right slightly then the picture changes.
\Cref{fig:.65Spike} shows how the positions change when $t_1=(.65\spikesep(T),0)$. The black circle $\partial B_{l_1}$, now with radius $.65\spikesep(T)$, pushes $t_2$, $t_3$, and $t_4$ out off the red circle, while the other points either move slightly closer or farther from the origin as the red circle moves to the right with $t_1$. In \Cref{fig:IntersectSpike} the nearest spike $t_1$ lies on the red line segment along the horizontal axis. Other $t_i$ must sit outside the intersection of circles along this segment (the red boundary) and $\partial B_{l_1}$ in black.
}
\end{figure}

Since $t_1$ sits on the line segment between $(l_1,0)$ and $(r_1,0)$, other spikes may not lie within $\spikesep(T)$ of that segment.
By \Cref{lem:ConvexIntersect} this is the set
\begin{equation}
C_1 := \{t:\norm{t-(l_1,0)}<\spikesep(T)\}\cap\{t:\norm{t-(r_1,0)}<\spikesep(T)\}.
\end{equation}
\Cref{fig:IntersectSpike} depicts this scenario where $t_1$ lies somewhere along the red line segment from $0.5\spikesep(T)$ to $0.8\spikesep(T)$ on the horizontal axis ($l_1=0.5\spikesep(T)$ and $r_1=0.8\spikesep(T)$).
$C_1$ is shaded in red, and denote the boundary of $C_1$ (shown as two red arcs) as $\partial C_1$.
The left and right arcs of $\partial C_1$ are parts of the borders of the disks of radius $\spikesep(T)$ centered at $(r_1,0)$ and $(l_1,0)$, respectively.
For each $i>1$, $t_i$ must lie in $U_i\setminus (C_1\cup B_{l_1})$.
%A lower bound for $\norm{t_i}$ is $\inf\{\norm{t}:t\in U_i\setminus (C_1\cup B_{l_1})\}$.
%is determined by the point in $U_i$ with smallest norm outside $C_1$ and farther than $l_1$.
By \Cref{lem:convmin}, we can lower bound $\|t_i\|$ by considering points on either $\partial C_1$ or $\partial B_{l_1}$.
We use this reasoning below to construct lower bounds on $\norm{t_i}$ for $i=5,\ldots,9$ while those for $i=2$, 3 and 4 are a slight modification, which we describe separately after.

\paragraph{$\norm{t_5}$, $\norm{t_6}$ bounds}\mbox{}

Since $B_{l_1}$ contains the point in $U_5$ nearest to the origin, we can apply \Cref{lem:convmin} to see the nearest point in $U_5\setminus (C_1\cup B_{l_1})$ either sits on $\partial B_{l_1}$ or $\partial C_1$.
The intersection of $\partial C_1$ with the vertical axis is $(y_1,y_2)=(0,\sqrt{\spikesep(T)^2-r_1^2})$, where $r_1\leq\Delta$ by assumption.
If $y_2>l_1$ then $U_5\cap B_{l_1}\subset U_5\cap C_1$.  To see this, note that
all points $(p_1,p_2)$ on the left arc of $\partial C_1$ in the first quadrant satisfy $0\leq p_1\leq\frac{l_1+r_1}{2}$ and $p_2\geq y_2$.  But all points $(q_1,q_2)$ on $\partial B_{l_1}$ in the first quadrant satisfy $0\leq q_1 \leq l_1$ and $q_2 \leq l_1< y_2$ proving the claim.
Thus we need only consider $\partial C_1$. The closest point on $\partial C_1\cap U_5$ to the origin is in fact $(0,y_2)$.  To see this, note that $C_1$ is symmetric about the line with first coordinate $\frac{l_1+r_1}{2}$.  Thus all $(p_1,p_2)$ on $\partial C_1$ with $0\leq p_1\leq l_1+r_1$ and $p_2>0$ satisfy $p_2\geq y_2$. But all points of $U_5$ have first coordinate less than $\frac{\sqrt{3}}{2}\spikesep(T)\leq l_1+r_1$ thus establishing \eqref{eq:t5t6}.

$U_6$ is a reflection of $U_5$ so $\norm{t_6}$ has the same bound. The reasoning for $\norm{t_7}$, $\norm{t_8}$ and $\norm{t_9}$ is similar, with details for their bounds given in \Cref{sec:t7t8} and \Cref{sec:t9}.

\paragraph{$\norm{t_3}$ bound}\mbox{}

For $\norm{t_2}$, $\norm{t_3}$ and $\norm{t_4}$ again note that $\norm{t_i}\geq\norm{t_1}\geq l_1$ since $t_1$ is the nearest spike.
Thus $t_2$, $t_3$ and $t_4$ lay outside the black circle $\partial B_{l_1}$ depicted in \Cref{fig:IntersectSpike}. %$l_1=\spikesep(T)/2$ is indicated by.
By assumption the first coordinate of $t_2$ lies in $[l_2,r_2]$ so $\norm{t_2}\geq\abs{r_2}$ as well, hence \eqref{eq:t2}.
%By considering how the location of $t_2$ constrains the possible locations for $t_3$, we will be able to improve our lower bound on $\|t_3\|$.

\begin{figure}[!t]
\begin{subfigure}[h]{0.5\textwidth}
\centering
\includegraphics{fig/LeftSpike.pdf}
\caption{\label{fig:LeftSpike}}
\end{subfigure}
\begin{subfigure}[h]{0.5\textwidth}
\centering
\includegraphics{fig/x2Left.pdf}
\caption{\label{fig:x2Left}}
\end{subfigure}
\caption[More Spike Perturbations]{
In \Cref{fig:LeftSpike}, $t_2$ lies in $P$ the blue region in $U_2$.
Then $t_3$ sits outside the solid blue arcs.
The interval for $t_1$ is indicated in red, while $t_4$ is shown outside $\partial B_{l_1}$ in black with radius $l_1=\norm{t_1}\leq\norm{t_1}$.
Dashed lines are circles of radius $\spikesep(T)$ about the upper vertices.
The red and green regions depict other possible regions for $P$ for different endpoints $l_2$ and $r_2$.
In \Cref{fig:x2Left}, the nearest possible positions from the origin for other spikes are shown when $t_1$ at $(.5\spikesep(T),0)$ and $t_2$ between $x=-.8\spikesep(T)$ and $x=-.5\spikesep(T)$.
}
\end{figure}

Let $P=U_2\cap\{(x_1,x_2):l_2\leq x_1\leq r_2, x_2\geq 0\}$. 
Since $P$ is a convex polygon, by \Cref{lem:ConvexIntersect} if $t_2$ lies in $P$ then $t_3$ must sit outside the region $C_2=\{y:\norm{y-x}<\spikesep(T)\ \forall x\in P\}=\{y:\norm{y-x}<\spikesep(T)\ \forall x\in\mbox{Vert}(P)\}$ where $\mbox{Vert}(P)$ are the vertices of $P$.
In \Cref{fig:LeftSpike} the three colored shapes are examples of choices of $P$.
Since $P$ has vertical sides, the points in $U_3$ within $\spikesep(T)$ of the bottom vertices are also within $\spikesep(T)$ of the top vertices.
This is true since, for $(u_1,u_2)\in U_3$, $u_2\geq\spikesep(T)/4$ so any top vertex $v=(v_1,v_2)$ of $P$ satisfies $\spikesep(T)/4\leq v_2\leq\spikesep(T)/2$ and the vertex below it would be $(v_1,0)$.
Hence $\abs{v_2-u_2}\leq\abs{u_2}$.
Thus $U_3\cap C_2=U_3\cap \{x:\norm{x-(l_2,0)}<\spikesep(T)\}\cap\{x:\norm{x-(r_2,0)}<\spikesep(T)\}$ which $t_3$ lies outside of.
Denote the boundary as $\partial C_2$, depicted in \Cref{fig:LeftSpike} by solid blue arcs.

%So $U_3\cap C_1=\{y\in U_3:\norm{y-x}\leq\spikesep(T)\forall x\in\mbox{Vert}(P)\}=\{y\in U_3:\norm{y-(l_2,0)}\leq\spikesep(T),\norm{y-(r_2,0)}\leq\spikesep(T)\}$ so points in $U_3$ outside of $C_1$.

$t_3$ is farther than the nearest point of $U_3\setminus(C_1\cup C_2\cup B_{l_1})$ which sits on either $\partial C_1$, $\partial C_2$ or $\partial B_{l_1}$ by \Cref{lem:convmin}.
Similar to $t_5$,
we get $\norm{t_3}\geq\max(l_1,\sqrt{\max(0,\spikesep(T)^2-l_2^2}))$ yielding \eqref{eq:t3a}.
\end{proof}

%%%%%%%APPENDIX MATERIAL%%%%%%%%%%

\section{Proofs for \Cref{lem:QBoundFar}}\label{sec:ProofsFarQBound}
\subsection{Proof of \Cref{lem:ConvexIntersect}}\label{sec:ConvexIntersectProof}

\ConvexIntersect*
\begin{proof}
Clearly $\bigcap_{c\in\conv\{a_i\}}S+c\subseteq\bigcap_i S+a_i$. Suppose $x\in\bigcap_{i=1}^n S+a_i$, and $c=\sum_{i=1}^n t_ia_i$ where $t_i\geq0$ and $\sum_i t_i=1$.
There exists $x_i\in S$ for each $i$ such that $x=x_i+a_i$. Thus $x=\sum_i t_i x=\sum_i t_i(x_i+a_i)=\sum_i t_i x_i+\sum_i t_i a_i=\sum_i t_i x_i+c$  and since $S$ is convex $\sum_it_ix_i\in S$.
Thus $x\in S+c$. Hence $\bigcap_{c\in\conv\{a_i\}}S+c=\bigcap_i S+a_i$.
\end{proof}

\subsection{Proof of \Cref{lem:convmin}}\label{sec:ConvMinProof}
\convmin*
\begin{proof}
If $v^*\notin B$ then the infimum achieves the minimum $\norm{v^*}^2$ on $A\setminus B$. Otherwise, suppose $v^\ast\in B$ and $a$ is any point in $A\setminus B$. Let $v_\partial$ be a point in $\partial B$ on the line segment between $v^\ast$ and $a$. Specifically, let $v_\partial=(1-t)v^\ast+ta\in \brac{\overline{A\setminus B}}\cap\partial B$
where
\begin{equation}
t = \inf\{s\in[0,1] : (1-s)v^\ast+sa \notin B\}.
\end{equation}
Then by convexity $\norm{ v_\partial}^2\leq (1-t)\norm{v^\ast}^2+t\norm{a}^2\leq (1-t)\norm{a}^2+t\norm{a}^2=\norm{a}^2$.  This proves that
\begin{equation}
    \inf_{v\in A\setminus B} \|v\|^2
    \geq \inf_{v\in\brac{\overline{A\setminus B}}\cap \partial B} \|v\|^2.
\end{equation}
But since every $v\in\brac{\overline{A\setminus B}}\cap \partial B$ is a limit point of $A\setminus B$, equality is obtained.
\end{proof}

\subsection{Remainder of \Cref{lem:Norms9}}

\begin{lemma}\label{lem:CircleDist}
Consider the points $y_\theta=(x+r\cos\theta,r\sin\theta)$ on the circle of radius $r$ centered at $(x,0)\in\RR^2$.  If $x>0$ then $\|y_\theta\|$ decreases for $\theta\in[0,\pi]$ and increases for $\theta\in[\pi,2\pi]$.  The reverse is true if $x<0$.
\end{lemma}
\begin{proof}
Note that $f(\theta):=\|y_\theta\|^2 = x^2+2xr\cos\theta+r^2$ has derivative $f'(\theta)=-2rx\sin\theta$.
\end{proof}

\subsubsection{$\norm{t_7}$, $\norm{t_8}$}\label{sec:t7t8}
For $\norm{t_7}$, again note that $C_1$ is the intersection of the two discs of radius $\spikesep$ about $l_1$ and $r_1$.
%, points $y=(y_1,y_2)$ such that $(y_1-l_1)^2+y_2^2=\spikesep^2$ and $(y_1-r_1)^2+y_2^2=\spikesep^2$.
By \Cref{lem:convmin,lem:CircleDist} the nearest point in $U_7\setminus C_1$ is the leftmost point of $\partial C_1$ in $U_7$ since $C_1$ contains the point of $U_7$ that is closest to the origin.
This is a point $y=(y_1,y_2)$ on the left edge of $U_7$ ($y_1=\sqrt{3}\spikesep/2$) and the arc $(y_1-l_1)^2+y_2^2=\spikesep^2$ if $(l_1+r_1)/2\leq\sqrt{3}\spikesep/2$, and on $(y_1-r_1)^2+y_2^2=\spikesep^2$ otherwise.
Thus we have that
\begin{equation}
\norm{t_7}\geq\norm{(y_1,y_2)}\mbox{ s.t. }y_1=\sqrt{3}\spikesep/2,\ y_2=
\begin{cases}
\sqrt{\spikesep^2-(\sqrt{3}\spikesep/2-l_1)^2} & \frac{l_1+r_1}{2}\leq\frac{\sqrt{3}\spikesep}{2},\\
\sqrt{\spikesep^2-(\sqrt{3}\spikesep/2-r_1)^2} & \frac{l_1+r_1}{2}\geq\frac{\sqrt{3}\spikesep}{2}.
\end{cases}
\end{equation}
Since $U_8$ is a reflection of $U_7$ across the horizontal axis $\norm{t_8}$ has the same bound.


% This occurs where $\partial C_1$ crosses the left edge of $U_7$ ($y_1=\sqrt{3}\spikesep/2$) since both $C_1$ and the left edge of $U_7$ have maximum possible height $\Delta$.  
% \bdb{I started changing this but I am confused.  Firstly, we are talking about crossing arcs but I don't think the arcs being described are well-defined.  Furthermore, why do we need a min?  Isn't this determined by whether $\sqrt{3}\spikesep/2 \geq \frac{l_1+r_1}{2}$?}
% ... the arc with coordinate $y_2$ smaller (crossing inside the other arc).
% Since $y_1=\sqrt{3}\spikesep/2$ then $y_2^2=\min\{\spikesep^2-(\sqrt{3}\spikesep/2-l_1)^2,\spikesep^2-(\sqrt{3}\spikesep/2-r_1)^2\}$ selects the point on the inner arc which is $\partial C_1$.

% and so the border $\partial C_1$ is determined by the arc with coordinate $y_2$ smaller in absolute value (i.e. inside the other circle).
% As before the nearest point in $U_7\setminus C_1$ is the leftmost point of $\partial C_1$ in $U_7$ which occurs where $\partial C_1$ crosses the vertical line $y_1=\sqrt{3}\spikesep/2$.
% Then $y_2^2=\min\{\spikesep^2-(\sqrt{3}\spikesep/2-l_1)^2,\spikesep^2-(\sqrt{3}\spikesep/2-r_1)^2\}$ selects the point on the inner arc which is $\partial C_1$.
% Thus we have that
% \begin{equation}
% \mbox{$\norm{t_7}\geq\sqrt{y_1^2+y_2^2}$ s.t. $y_1=\sqrt{3}\spikesep/2,\ y_2^2=\min\{\spikesep^2-(\sqrt{3}\spikesep/2-l_1)^2,\spikesep^2-(\sqrt{3}\spikesep/2-r_1)^2\}$}.
% \end{equation}
% Since $U_8$ is a reflection of $U_7$ across the horizontal axis $\norm{t_8}$ has the same bound.

\subsubsection{$\norm{t_9}$}\label{sec:t9}
By \Cref{lem:convmin,lem:CircleDist} the nearest point in $U_9\setminus C_1$
is on $\partial C_1's$ right arc, points $(y_1,y_2)$ such that $(y_1-l_1)^2+y_2^2=\spikesep^2$, at its leftmost point by \Cref{lem:CircleDist} (the left arc will not intersect $U_9$).
We consider this in the upper plane, as the lower is symmetric and has the same bound.
If $l_1\leq \sqrt{3}\spikesep/2$ then the right arc crosses the top left edge $y_2=\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2}$, and otherwise crosses the top right $y_2=-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}$.
Thus,
\begin{equation}
\norm{t_9}\geq\norm{(y_1,y_2)}\ \mbox{s.t.}\ (y_1-l_1)^2+y_2^2=\spikesep^2\ \mbox{and}\ y_2=
\begin{cases}
\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2} & l_1\leq \frac{\sqrt{3}\spikesep}{2},\\
-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2} & l_1\geq \frac{\sqrt{3}\spikesep}{2}.
\end{cases}
\end{equation}


% \bdb{Instead of referring to the figure and talking about closeness we should be precise on the conditions for each crossing.  Also, I don't see why we are taking a min.  Again, isn't this uniquely determined by the value of $l_1$, which we know a priori?}
% Looking at \Cref{fig:IntersectSpike} we see that if $l_1$ is close to $\spikesep/2$, the right arc crosses the top left edge of $U_9$, a segment of the line $y_2=\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2}$.
% But for $l_1$ closer to $\spikesep$ the arc instead crosses $U_9$'s top right edge, a portion of the line $y_2=-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}$.
% Since the minimum of both lines gives these two edges the $y_2$ coordinate is given by $y_2=\min\{\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2},-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}\}$.
% Thus,
% \begin{equation}
% \mbox{$\norm{t_9}\geq\sqrt{y_1^2+y_2^2}$ s.t. $(y_1-l_1)^2+y_2^2=\spikesep^2$ and $y_2=\min\{\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2},-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}\}$}.
% \end{equation}

% \subsubsection{$B_{z_1}\subset C_1\cup C_2$}
% \begin{lemma}\label{lem:BZ1}
% $B_{z_1}\subset C_1\cup C_2$.
% \end{lemma}
% \begin{proof}
% $\partial B_{z_1}$ satisfies $x_2^2=z_1^2+z_2^2-x_1^2$, $\partial C_1$ satisfies $x_2^2=(r_1-z_1)^2+z_2^2-(r_1-x_1)^2$ and $\partial C_2$ satisfies $x_2^2=(l_2-z_1)^2+z_2^2-(l_2-x_1)^2$ for $(x_1,x_2)$ on their curves with $l_2\leq 0\leq r_1$.
% If $x_1\geq z_1$ then 
% \begin{align}
% z_1^2+z_2^2-x_1^2&\leq z_1^2+z_2^2-x_1^2+2r_1(x_1-z_1)\\
% &=(r_1-z_1)^2+z_2^2-(r_1-x_1)^2
% \end{align}
% since $r_1>0$. If $x_1\leq z_1$ then 
% \begin{align}
% z_1^2+z_2^2-x_1^2&\leq z_1^2+z_2^2-x_1^2+2l_2(x_1-z_1)\\
% &=(l_2-z_1)^2+z_2^2-(l_2-x_1)^2
% \end{align}
% since $l_2<0$. Since the top arc of $B_{z_1}$ is underneath either arc of $C_1$ and $C_2$ it is contained in them,

% For $r_2$
% \end{proof}


% In both cases, by \Cref{lem:CircleDist} the point of $U_9\setminus C_1$ nearest to the origin is $\partial C_1$'s leftmost point on those lines:
% \begin{equation}
% \mbox{$\norm{t_9}\geq\sqrt{y_1^2+y_2^2}$ s.t. $(y_1-l_1)^2+y_2^2=\spikesep^2$ and $y_2=\min\{\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2},-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}\}$}.
% \end{equation}


% lies outside $\partial C_1$'s right arc or points $y=(y_1,y_2)$ where $\norm{y-(l_1,0)}^2=(y_1-l_1)^2+y_2^2=\spikesep^2$ (with radius $\spikesep$ about the left endpoint).
% $U_9$ and $\partial C_1$ are symmetric across the horizontal axis so two equally close points sitting above and below the axis are reflections of each other, so in both cases their distances are the same.
% Looking at \Cref{fig:IntersectSpike} we see that if $l_1$ is close to $\spikesep/2$, the right arc crosses the top left edge of $U_9$, a segment of the line $y_2=\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2}$.
% But for $l_1$ closer to $\spikesep$ the arc instead crosses $U_9$'s top right edge, a portion of the line $y_2=-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}$.
% In both cases, by \Cref{lem:CircleDist} the point of $U_9\setminus C_1$ nearest to the origin is $\partial C_1$'s leftmost point on those lines:
% \begin{equation}
% \mbox{$\norm{t_9}\geq\sqrt{y_1^2+y_2^2}$ s.t. $(y_1-l_1)^2+y_2^2=\spikesep^2$ and $y_2=\min\{\frac{y_1}{\sqrt{3}}-\frac{\spikesep}{2},-\frac{y_1}{\sqrt{3}}+\frac{3\spikesep}{2}\}$}.
% \end{equation}













